Crust Cooling Models are Insensitive to the Crust-Core Transition Pressure for Realistic Equations of State

Neutron stars cooling after sustained accretion outbursts provide unique information about the neutron star crust and underlying dense matter. Comparisons between astronomical observations of these cooling transients and model calculations of neutron star crust cooling have frequently been used to constrain neutron star properties such as the mass, radius, crust composition, and presence of nuclear pasta. These calculations often use a fixed pressure at which the crust-core transition happens, though this quantity depends on the dense matter equation of state. We demonstrate that varying the crust-core transition pressure in a manner consistent with adopting various equations of state results in modest changes to the crust cooling light curve. This validates the approach adopted in most crust cooling studies to date, where the neutron star mass and radius are varied while leaving the crust-core transition pressure constant.

==> st_code.tex <==
% code.tex
% Edward F Brown, Michigan State University
% 
% Macros for commonly used codes
% 
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\flash}{FLASH}
\newcommand{\kepler}{KEPLER}
\newcommand{\nonsmoker}{NON-SMOKER}
\newcommand{\mesa}{\code{MESA}}
\newcommand{\MESA}{\mesa}
\newcommand{\STERN}{STERN}
\newcommand{\ADIPLS}{\code{ADIPLS}}
\newcommand{\DSEP}{DSEP}
\newcommand{\enzo}{\code{ENZO}}
\newcommand{\dStar}{\code{dStar}}
\newcommand{\netJina}{\code{netJina}}
\newcommand{\starType}{\code{starType}}
\newcommand{\AMReX}{\code{AMReX}}
\newcommand{\BoxLib}{\code{BoxLib}}
\newcommand{\Castro}{\code{Castro}}
\newcommand{\Maestro}{\code{Maestro}}
\newcommand{\amrex}{\AMReX}
\newcommand{\boxlib}{\BoxLib}
\newcommand{\castro}{\Castro}
\newcommand{\maestro}{\Maestro}



==> st_derivatives.tex <==
% derivatives.tex
% Edward F Brown, Michigan State University
% 
% typesetting of common derivatives

\newcommand*{\dif}{\ensuremath{\mathrm{d}}}  % differential operator, roman typeface
\newcommand*{\Dif}{\ensuremath{\mathrm{D}}} % lagrangian differential operator
\newcommand*{\jac}[4]{\ensuremath{\frac{\partial(#1,#2)}{\partial(#3,#4)}}} %jacobian
\newcommand*{\tderiv}[3]{\ensuremath{\left(\frac{\partial #1}{\partial #2}\right)_{#3}}} %thermodynamic derivative

%derivatives
\newcommand*{\ddt}[1]{\frac{\partial #1}{\partial t}}    % partial time derivative 
\newcommand*{\DDt}[1]{\frac{\dif #1}{\dif t}}            % total time derivative
\newcommand*{\ddx}[1]{\frac{\partial #1}{\partial x}}    % partial derivative wrt x 
\newcommand*{\DDx}[1]{\frac{\dif #1}{\dif x}}            % total derivative wrt x
\newcommand*{\ddy}[1]{\frac{\partial #1}{\partial y}}    % partial derivative wrt y 
\newcommand*{\DDy}[1]{\frac{\dif #1}{\dif y}}            % total derivative wrt y
\newcommand*{\ddz}[1]{\frac{\partial #1}{\partial z}}    % partial derivative wrt z 
\newcommand*{\DDz}[1]{\frac{\dif #1}{\dif z}}            % total derivative wrt z

\newcommand*{\DD}[2]{\frac{\dif #1}{\dif #2}}           % total derivative
\newcommand*{\dd}[2]{\frac{\partial #1}{\partial #2}}           % partial derivative


==> st_nuclides.tex <==
% nuclides.tex
% Edward F. Brown, Michigan State University
%
% input file with macros for nuclides

% base command
\newcommand*{\nuclei}[2]{\ensuremath{\mathrm{^{#1}#2}}}

% nuclides, with most highest abundance or longest half-life as default
% for example, \carbon produces ^{12}C, \carbon[13] produces ^{13}C
%
\newcommand*{\neutron}{\ensuremath{\mathrm{n}}}
\newcommand*{\nt}{\neutron}
\newcommand*{\proton}{\ensuremath{\mathrm{p}}}
\newcommand*{\pt}{\proton}
\newcommand*{\hydrogen}[1][1]{\nuclei{#1}{H}}
\newcommand*{\helium}[1][4]{\nuclei{#1}{He}}
\newcommand*{\lithium}[1][7]{\nuclei{#1}{Li}}
\newcommand*{\beryllium}[1][9]{\nuclei{#1}{Be}}
\newcommand*{\boron}[1][11]{\nuclei{#1}{B}}
\newcommand*{\carbon}[1][12]{\nuclei{#1}{C}}
\newcommand*{\nitrogen}[1][14]{\nuclei{#1}{N}}
\newcommand*{\oxygen}[1][16]{\nuclei{#1}{O}}
\newcommand*{\fluorine}[1][19]{\nuclei{#1}{F}}
\newcommand*{\neon}[1][20]{\nuclei{#1}{Ne}}
\newcommand*{\sodium}[1][23]{\nuclei{#1}{Na}}
\newcommand*{\magnesium}[1][24]{\nuclei{#1}{Mg}}
\newcommand*{\aluminum}[1][27]{\nuclei{#1}{Al}}
\newcommand*{\silicon}[1][28]{\nuclei{#1}{Si}}
\newcommand*{\phosphorus}[1][31]{\nuclei{#1}{P}}
\newcommand*{\sulfur}[1][32]{\nuclei{#1}{S}}
\newcommand*{\chlorine}[1][35]{\nuclei{#1}{Cl}}
\newcommand*{\argon}[1][36]{\nuclei{#1}{Ar}}
\newcommand*{\potassium}[1][39]{\nuclei{#1}{K}}
\newcommand*{\calcium}[1][40]{\nuclei{#1}{Ca}}
\newcommand*{\scandium}[1][45]{\nuclei{#1}{Sc}}
\newcommand*{\titanium}[1][48]{\nuclei{#1}{Ti}}
\newcommand*{\vanadium}[1][51]{\nuclei{#1}{V}}
\newcommand*{\chromium}[1][52]{\nuclei{#1}{Cr}}
\newcommand*{\manganese}[1][55]{\nuclei{#1}{Mn}}
\newcommand*{\iron}[1][56]{\nuclei{#1}{Fe}}
\newcommand*{\cobalt}[1][59]{\nuclei{#1}{Co}}
\newcommand*{\nickel}[1][58]{\nuclei{#1}{Ni}}
\newcommand*{\copper}[1][63]{\nuclei{#1}{Cu}}
\newcommand*{\zinc}[1][64]{\nuclei{#1}{Zn}}
\newcommand*{\gallium}[1][69]{\nuclei{#1}{Ga}}
\newcommand*{\germanium}[1][74]{\nuclei{#1}{Ge}}
\newcommand*{\arsenic}[1][75]{\nuclei{#1}{As}}
\newcommand*{\selenium}[1][80]{\nuclei{#1}{Se}}
\newcommand*{\bromine}[1][79]{\nuclei{#1}{Br}}
\newcommand*{\krypton}[1][84]{\nuclei{#1}{Kr}}
\newcommand*{\rubidium}[1][85]{\nuclei{#1}{Rb}}
\newcommand*{\strontium}[1][88]{\nuclei{#1}{Sr}}
\newcommand*{\yttrium}[1][89]{\nuclei{#1}{Y}}
\newcommand*{\zirconium}[1][94]{\nuclei{#1}{Zr}}
\newcommand*{\niobium}[1][93]{\nuclei{#1}{Nb}}
\newcommand*{\molybdenum}[1][98]{\nuclei{#1}{Mo}}
\newcommand*{\technetium}[1][97]{\nuclei{#1}{Tc}}
\newcommand*{\ruthenium}[1][102]{\nuclei{#1}{Ru}}
\newcommand*{\rhodium}[1][103]{\nuclei{#1}{Rh }}
\newcommand*{\palladium}[1][106]{\nuclei{#1}{Pd}}
\newcommand*{\silver}[1][107]{\nuclei{#1}{Ag}}
\newcommand*{\cadmium}[1][114]{\nuclei{#1}{Cd}}
\newcommand*{\indium}[1][115]{\nuclei{#1}{In}}
\newcommand*{\tin}[1][120]{\nuclei{#1}{Sn}}
\newcommand*{\antimony}[1][121]{\nuclei{#1}{Sb}}
\newcommand*{\tellurium}[1][130]{\nuclei{#1}{Te}}
\newcommand*{\iodine}[1][127]{\nuclei{#1}{I}}
\newcommand*{\xenon}[1][132]{\nuclei{#1}{Xe}}
\newcommand*{\cesium}[1][133]{\nuclei{#1}{Cs}}
\newcommand*{\barium}[1][138]{\nuclei{#1}{Ba}}
\newcommand*{\lanthanum}[1][139]{\nuclei{#1}{La}}
\newcommand*{\cerium}[1][140]{\nuclei{#1}{Ce}}
\newcommand*{\praseodymium}[1][141]{\nuclei{#1}{Pr}}
\newcommand*{\neodymium}[1][142]{\nuclei{#1}{Nd}}
\newcommand*{\promethium}[1][147]{\nuclei{#1}{Pm}}
\newcommand*{\samarium}[1][152]{\nuclei{#1}{Sm}}
\newcommand*{\europium}[1][153]{\nuclei{#1}{Eu}}
\newcommand*{\gadolinium}[1][158]{\nuclei{#1}{Gd}}
\newcommand*{\terbium}[1][159]{\nuclei{#1}{Tb}}
\newcommand*{\dysprosium}[1][164]{\nuclei{#1}{Dy}}
\newcommand*{\holmium}[1][165]{\nuclei{#1}{Ho}}
\newcommand*{\erbium}[1][168]{\nuclei{#1}{Er}}
\newcommand*{\thulium}[1][169]{\nuclei{#1}{Tm}}
\newcommand*{\ytterbium}[1][174]{\nuclei{#1}{Yb}}
\newcommand*{\lutetium}[1][175]{\nuclei{#1}{Lu}}
\newcommand*{\hafnium}[1][180]{\nuclei{#1}{Hf}}
\newcommand*{\tantalum}[1][180]{\nuclei{#1}{Ta}}
\newcommand*{\tungsten}[1][184]{\nuclei{#1}{W}}
\newcommand*{\rhenium}[1][187]{\nuclei{#1}{Re}}
\newcommand*{\osmium}[1][192]{\nuclei{#1}{Os}}
\newcommand*{\iridium}[1][193]{\nuclei{#1}{Ir}}
\newcommand*{\platnium}[1][195]{\nuclei{#1}{Pt}}
\newcommand*{\gold}[1][197]{\nuclei{#1}{Au}}
\newcommand*{\mercury}[1][202]{\nuclei{#1}{Hg}}
\newcommand*{\thallium}[1][205]{\nuclei{#1}{Tl}}
\newcommand*{\lead}[1][208]{\nuclei{#1}{Pb}}
\newcommand*{\bisumth}[1][209]{\nuclei{#1}{Bi}}
\newcommand*{\polonium}[1][210]{\nuclei{#1}{Po}}
\newcommand*{\astatine}[1][210]{\nuclei{#1}{At}}
\newcommand*{\radon}[1][222]{\nuclei{#1}{Rn}}
\newcommand*{\francium}[1][223]{\nuclei{#1}{Fr}}
\newcommand*{\radium}[1][226]{\nuclei{#1}{Ra}}
\newcommand*{\actinium}[1][227]{\nuclei{#1}{Ac}}
\newcommand*{\thorium}[1][232]{\nuclei{#1}{Th}}
\newcommand*{\protactinium}[1][231]{\nuclei{#1}{Pa}}
\newcommand*{\uranium}[1][238]{\nuclei{#1}{U}}
\newcommand*{\neptunium}[1][237]{\nuclei{#1}{Np}}
\newcommand*{\plutonium}[1][244]{\nuclei{#1}{Pu}}
\newcommand*{\americium}[1][243]{\nuclei{#1}{Am}}
\newcommand*{\curium}[1][247]{\nuclei{#1}{Cm}}
\newcommand*{\berkelium}[1][247]{\nuclei{#1}{Bk}}
\newcommand*{\californium}[1][251]{\nuclei{#1}{Cf}}
\newcommand*{\einsteinium}[1][252]{\nuclei{#1}{Es}}
\newcommand*{\fermium}[1][257]{\nuclei{#1}{Fm}}
\newcommand*{\mendelevium}[1][258]{\nuclei{#1}{Md}}
\newcommand*{\nobelium}[1][259]{\nuclei{#1}{No}}
\newcommand*{\lawrencium}[1][262]{\nuclei{#1}{Lr}}
\newcommand*{\rutherfordium}[1][261]{\nuclei{#1}{Rf}}
\newcommand*{\dubnium}[1][268]{\nuclei{#1}{Db}}
\newcommand*{\seaborgium}[1][271]{\nuclei{#1}{Sg}}
\newcommand*{\bohrium}[1][274]{\nuclei{#1}{Bh}}
\newcommand*{\hassium}[1][270]{\nuclei{#1}{Hs}}
\newcommand*{\meitnerium}[1][278]{\nuclei{#1}{Mt}}
\newcommand*{\darmstadtium}[1][281]{\nuclei{#1}{Ds}}
\newcommand*{\roentgenium}[1][281]{\nuclei{#1}{Rg}}
\newcommand*{\copernicum}[1][285]{\nuclei{#1}{Cn}}


==> st_symbols.tex <==
% symbols.tex
% Edward Brown, Michigan State University
%
% symbols for commonly used expressions in stellar astrophysics.


\newcommand*{\epsnuc}{\ensuremath{\epsilon_{\mathrm{nuc}}}}	% nuclear heating rate
\newcommand*{\epsgrav}{\ensuremath{\epsilon_{\mathrm{grav}}}} % gravitational heating rate
\newcommand*{\epsnu}{\ensuremath{\epsilon_{\mathrm{\nu}}}} % neutrino losses
\newcommand*{\Teff}{\ensuremath{T_{\!\mathrm{eff}}}}	% effective temperature
\newcommand*{\teff}{\Teff}
\newcommand*{\Ledd}{\ensuremath{L_{\mathrm{Edd}}}} % Eddington Luminosity
\newcommand*{\logg}{\ensuremath{\log g}}	% log surface gravity
\newcommand*{\Tc}{\ensuremath{T_{\mathrm{\!c}}}} % central temperature
\newcommand*{\Pc}{\ensuremath{P_{\mathrm{\!c}}}} % central pressure
\newcommand*{\rhoc}{\ensuremath{\rho_{\mathrm{c}}}} % central density
\newcommand*{\CP}{\ensuremath{C_{\!P}}} % specific heat at constant pressure
\newcommand*{\Mdot}{\ensuremath{\dot{M}}} % mass-loss rate

% for correction between baryon densities and mass-energy densities
\newcommand*{\nB}{\ensuremath{n_{\mathrm{B}}}}	% baryon density

% thermodynamical Gammas
\newcommand*{\Gammaone}{\ensuremath{\Gamma_{\!1}}} % $ (\partial\ln P/\partial \ln\rho)_S$
\newcommand*{\Gammatwo}{\ensuremath{\Gamma_{\!2}}} % $ \left[1-(\partial\ln T/\partial\ln P)_S\right]^{-1}$
\newcommand*{\Gammathree}{\ensuremath{\Gamma_{\!3}}} % $ 1+ (\partial\ln T/\partial\ln\rho)_S$

% stellar gradients
\newcommand*{\alphaMLT}{\ensuremath{\alpha_{\mathrm{MLT}}}}	% mixing length parameter
\newcommand*{\chirho}{\ensuremath{\chi_{\rho}}}	% $(\partial\ln P/\partial\ln\rho)_T$
\newcommand*{\chiT}{\ensuremath{\chi_{\raisebox{-2pt}{$\scriptstyle T$}}}}	% $(\partial\ln P/\partial\ln T)_{\rho}$
\newcommand*{\Dov}{\ensuremath{D_{\mathrm{ov}}}}	% overshoot diffusion coefficient
\newcommand*{\nablaad}{\ensuremath{\nabla_{\!\mathrm{ad}}}}	% adiabatic temperature gradient
\newcommand*{\nablarad}{\ensuremath{\nabla_{\!\mathrm{rad}}}}	% radiative temperature gradient
\newcommand*{\nablaT}{\ensuremath{\nabla_{\!T}}}	% actual temperature gradient
\newcommand*{\nablaL}{\ensuremath{\nabla_{\mathrm{\!L}}}}	% Ledoux criterion
\newcommand*{\scaleheight}{\ensuremath{\lambda_P}}	% pressure scale height
\newcommand*{\Pgas}{\ensuremath{P_{\!\!\mathrm{gas}}}}	% gas pressure

% more symbols for radiation and gas pressures
\newcommand*{\Prad}{\ensuremath{P_{\!\!\mathrm{rad}}}}	% radiation pressure
\newcommand*{\Lrad}{\ensuremath{L_{\mathrm{rad}}}}	% radiative luminosity
\newcommand*{\Fconv}{\ensuremath{F_{\!\mathrm{conv}}}}		% convective flux
\newcommand*{\Frad}{\ensuremath{F_{\!\mathrm{rad}}}}	% radiative flux

% mixing symbols
\newcommand*{\alphasc}{\ensuremath{\alpha_{\mathrm{sc}}}} % semiconvection efficiency parameter
\newcommand*{\alphath}{\ensuremath{\alpha_{\mathrm{th}}}} % thermohaline efficiency parameter
\newcommand*{\Dth}{\ensuremath{D_{\mathrm{th}}}} % thermohaline diffusion coefficient
\newcommand*{\fov}{\ensuremath{f_{\mathrm{ov}}}} % convective overshoot parameter

% physical constants
\newcommand*{\kB}{\ensuremath{k_\mathrm{B}}} % Boltzmann constant
\newcommand*{\NA}{\ensuremath{N_\mathrm{\!A}}} % Avogadro number
\newcommand*{\mb}{\ensuremath{m_\mathrm{u}}} % atomic mass unit
\newcommand*{\sigmaSB}{\ensuremath{\sigma_\mathrm{\!SB}}} % Stefan-Boltzmann constant
\newcommand*{\pF}{\ensuremath{p_\mathrm{F}}} %Fermi momentum
\newcommand*{\EF}{\ensuremath{E_\mathrm{F}}} %Fermi energy
\newcommand*{\me}{\ensuremath{m_\mathrm{e}}} %electron mass
\newcommand*{\mpr}{\ensuremath{m_\mathrm{p}}} %proton mass
\newcommand*{\mn}{\ensuremath{m_\mathrm{n}}} %neutron mass
\newcommand*{\alphaF}{\ensuremath{\alpha}} %Fine structure
\newcommand*{\lambdaD}{\ensuremath{\lambda_{\mathrm{D}}}} %Debye length
\newcommand*{\abohr}{\ensuremath{a_{\mathrm{B}}}} %Bohr radius


% stellar parameters
\newcommand*{\tkh}{\ensuremath{\tau_{\mathrm{KH}}}} % thermal (Kelvin-Helmholtz) timescale

% asteroseismology
\newcommand*{\cs}{\ensuremath{c_{\rm s}}} % adiabatic sound speed
\newcommand*{\Slamb}{\ensuremath{S_{\!\ell}}} % Lamb frequency

% fluids, dimensionless numbers
\newcommand*{\fluidnumber}[1]{\ensuremath{\mathrm{#1}}}
\newcommand*{\Ma}{\fluidnumber{Ma}}	% Mach number
\newcommand*{\Rey}{\fluidnumber{Re}}	% Reynolds number
\newcommand*{\Da}{\fluidnumber{Da}} % Damk\"ohler number
\newcommand*{\lG}{\ensuremath{\ell_{\mathrm{G}}}} % Gibson length



==> st_units.tex <==
% units.tex
% Edward F Brown, Michigan State University
% 
% typesetting of dimensional values
% Features: proper spacing between value and unit; unit is set in correct type

% powers
\newcommand*{\ee}[1]{\ensuremath{\times 10^{#1}}}		% 3.0\ee{4} => 3.0\times 10^{4}
\newcommand*{\sci}[2]{\ensuremath{#1\ee{#2}}}			% \sci{3.0}{4} => 3.0\times 10^{4}
\newcommand{\power}[2]{\ensuremath{{#1}^{#2}}}		    % \power{2}{3} => 2^{3}

% spacing between value and unit; value is a thin space
\newcommand*{\unitskip}{\,}                             % change this to \; if you want a thicker space
\newcommand*{\usk}{\unitskip}
\newcommand*{\val}[2]{\ensuremath{#1\unitskip#2}}

% sometimes you want to input a range of numbers
% example: \rng{2}{3} puts 2 to 3; \rng[--]{2}{3} puts 2--3, where the two dashes are correctly typeset 
% as an en-dash rather than as a minus sign
\newcommand*{\rng}[3][~to~]{\ensuremath{#2\textrm{#1}#3}}
% this puts in a range with a unit
% example: \valrng[--]{2}{3}{\times \val{10^{3}}{\kilo\gram}}
\newcommand*{\valrng}[4][~to~]{\ensuremath{\left(#2\textrm{#1}#3\right)#4}}


% units should be in upright (roman) font
\newcommand*{\unitstyle}[1]{\mathrm{#1}}

% pre-defined macros for common units
% prefixes
\newcommand*{\yocto}{\unitstyle{y}}		% 10^{-24}
\newcommand*{\zepto}{\unitstyle{z}}		% 10^{-21}
\newcommand*{\atto}{\unitstyle{a}}		% 10^{-18}
\newcommand*{\femto}{\unitstyle{f}}		% 10^{-15}
\newcommand*{\pico}{\unitstyle{p}}		% 10^{-12}
\newcommand*{\nano}{\unitstyle{n}}		% 10^{-9}
\newcommand*{\micro}{\unitstyle{\mu}}	% 10^{-6}
\newcommand*{\milli}{\unitstyle{m}}		% 10^{-3}
\newcommand*{\centi}{\unitstyle{c}}		% 10^{-2}
\newcommand*{\deci}{\unitstyle{d}}		% 10^{-1}
%
\newcommand*{\deka}{\unitstyle{da}}		% 10^{1}
\newcommand*{\hecto}{\unitstyle{h}}		% 10^{2}
\newcommand*{\kilo}{\unitstyle{k}}		% 10^{3}
\newcommand*{\Mega}{\unitstyle{M}}		% 10^{6}
\newcommand*{\Giga}{\unitstyle{G}}		% 10^{9}
\newcommand*{\Tera}{\unitstyle{T}}		% 10^{12}
\newcommand*{\Peta}{\unitstyle{P}}		% 10^{15}
\newcommand*{\Exa}{\unitstyle{E}}		% 10^{18}
\newcommand*{\Zetta}{\unitstyle{Z}}		% 10^{21}
\newcommand*{\Yotta}{\unitstyle{Y}}		% 10^{24}

% base units, mks
\newcommand*{\meter}{\unitstyle{m}}
\newcommand*{\kilogram}{\kilo\gram}
\newcommand*{\second}{\unitstyle{s}}

\newcommand*{\Kelvin}{\unitstyle{K}}
\newcommand*{\K}{\Kelvin}  %degrees Kelvin

% base units, cgs
\newcommand*{\cm}{\centi\meter}
\newcommand*{\gram}{\unitstyle{g}}

% derived units
\newcommand*{\grampercc}{\gram\unitskip\power{\cm}{-3}} %mass density
\newcommand*{\grampersquarecm}{\gram\unitskip\power{\cm}{-2}} %column depth
\newcommand*{\GramPerCc}{\grampercc}
\newcommand*{\GramPerSc}{\grampersquarecm}
\newcommand*{\columnunit}{\grampersquarecm}
\newcommand*{\dyne}{\unitstyle{dyn}}            %dyne
\newcommand*{\erg}{\unitstyle{erg}}             %ergs
\newcommand*{\ergs}{\erg}
\newcommand*{\gauss}{\unitstyle{G}}             %gauss
\newcommand*{\ergspersecond}{\erg\unitskip\power{\second}{-1}}
\newcommand*{\ergspergram}{\erg\unitskip\power{\gram}{-1}}
\newcommand*{\cgsflux}{\erg\unitskip\power{\cm}{-2}\unitskip\power{\second}{-1}}

% Nuclear and atomic units
\newcommand*{\amu}{\unitstyle{u}}               %atomic mass unit
\newcommand*{\angstrom}{\mbox{\AA}}             %Angstrom
\newcommand*{\fermi}{\femto\meter}              %fermi
\newcommand*{\eV}{\unitstyle{eV}}               %eV
\newcommand*{\keV}{\kilo\eV}                    %keV
\newcommand*{\MeV}{\Mega\eV}                    %MeV
\newcommand*{\GeV}{\Giga\eV}                    %GeV
% Beam units
\newcommand*{\MeVA}{\MeV/A}                     % MeV per nucleon
\newcommand*{\GeVA}{\GeV/A}                     % GeV per nucleon

% misc. units
\newcommand*{\minute}{\unitstyle{min}}          %minute
\newcommand*{\hour}{\unitstyle{hr}}             %hour
\newcommand*{\yr}{\unitstyle{yr}}               %year
\newcommand*{\km}{\kilo\meter}                  %kilometers
\newcommand*{\Hz}{\unitstyle{Hz}}               %Hertz
\newcommand*{\ksec}{\kilo\second}               %kilosecond
\newcommand*{\mol}{\unitstyle{mol}}             % mole
\newcommand*{\barn}{\ensuremath{\mathrm{b}}}    %barn

% solar and astronomical units
\newcommand*{\Msun}{\ensuremath{M_\odot}}
\newcommand*{\Lsun}{\ensuremath{L_\odot}}
\newcommand*{\Rsun}{\ensuremath{R_\odot}}
\newcommand*{\Myr}{\Mega\yr}
\newcommand*{\Gyr}{\Giga\yr}
\newcommand*{\AU}{\unitstyle{AU}}               % astronomical unit
\newcommand*{\parsec}{\unitstyle{pc}}           % parsec
\newcommand*{\kpc}{\kilo\parsec}                % kiloparsec
\newcommand*{\Jansky}{\unitstyle{Jy}}           % Jansky
\newcommand*{\mJy}{\unitstyle{\mu Jy}}          % micro Jansky
\newcommand*{\Msunperyr}{\Msun\unitskip\power{\yr}{-1}}	% solar masses per year


==> st_vectors.tex <==
% vectors.tex
% Edward Brown, Michigan State University
%
% Some basic vector operators
%
% Requires package bm.sty
%

\RequirePackage{bm}
\newcommand{\bvec}[1]{\ensuremath{\bm{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\bm{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}

